GPEX, A Framework For Interpreting Artificial Neural Networks

The analogy between Gaussian processes (GPs) and deep artificial neural networks (ANNs) has received a lot of interest, and has shown promise to unbox the blackbox of deep ANNs. Existing theoretical works put strict assumptions on the ANN (e.g. requiring all intermediate layers to be wide, or using specific activation functions). Accommodating those theoretical assumptions is hard in recent deep architectures, and those theoretical conditions need refinement as new deep architectures emerge. In this paper we derive an evidence lower-bound that encourages the GP's posterior to match the ANN's output without any requirement on the ANN. Using our method we find out that on 5 datasets, only a subset of those theoretical assumptions are sufficient. Indeed, in our experiments we used a normal ResNet-18 or feed-forward backbone with a single wide layer in the end. One limitation of training GPs is the lack of scalability with respect to the number of inducing points. We use novel computational techniques that allow us to train GPs with hundreds of thousands of inducing points and with GPU acceleration. As shown in our experiments, doing so has been essential to get a close match between the GPs and the ANNs on 5 datasets. We implement our method as a publicly available tool called GPEX: https://github.com/amirakbarnejad/gpex. On 5 datasets (4 image datasets, and 1 biological dataset) and ANNs with 2 types of functionality (classifier or attention-mechanism) we were able to find GPs whose outputs closely match those of the corresponding ANNs. After matching the GPs to the ANNs, we used the GPs' kernel functions to explain the ANNs' decisions. We provide more than 200 explanations (around 30 explanations in the paper and the rest in the supplementary) which are highly interpretable by humans and show the ability of the obtained GPs to unbox the ANNs' decisions.

==> TexSubfigs/test_subfig.tex <==
\begin{figure*}
    \captionsetup[subfigure]{labelformat=empty}
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:1}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:2}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:3}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:4}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:5}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:6}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:7}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:8}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:9}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:10}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:11}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:12}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:13}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:14}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:15}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:16}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:17}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:18}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:19}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:20}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:21}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:22}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:23}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:24}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:25}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:26}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:27}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:28}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:29}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:30}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:31}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:32}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:33}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:34}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:35}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:36}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:37}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:38}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:39}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:40}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:41}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:42}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:43}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:44}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:45}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:46}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:47}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:48}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:49}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:50}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:51}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:52}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:53}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:54}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:55}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:56}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:57}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:58}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:59}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:60}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:61}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:62}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:63}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:64}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:65}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:66}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:67}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:68}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:69}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:70}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:71}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:72}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:73}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:74}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:75}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:76}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:77}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:78}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:79}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:80}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:81}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:82}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:83}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:84}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:85}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:86}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:87}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:88}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:89}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:90}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:91}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:92}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:93}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:94}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:95}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:96}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:97}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:98}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:99}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.095\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/sample.png}
            \label{fig:100}
        \end{subfigure}
    \caption[]
    {Some captions}
    \label{fig:label}
\end{figure*}

==> Texfiles_ToInput/DogsWolves/dogswolves_0_11_mainarticle.tex <==
\begin{figure*}
    \captionsetup[subfigure]{labelformat=empty}
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/45/instance.png}
            \label{fig:kather_10NN_1}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/45/1.png}
            \label{fig:kather_10NN_2}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/45/2.png}
            \label{fig:kather_10NN_3}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/45/3.png}
            \label{fig:kather_10NN_4}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/45/4.png}
            \label{fig:kather_10NN_5}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/45/5.png}
            \label{fig:kather_10NN_6}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/45/6.png}
            \label{fig:kather_10NN_7}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/45/7.png}
            \label{fig:kather_10NN_8}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/45/8.png}
            \label{fig:kather_10NN_9}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/45/9.png}
            \label{fig:kather_10NN_10}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/45/10.png}
            \label{fig:kather_10NN_11}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/56/instance.png}
            \label{fig:kather_10NN_12}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/56/1.png}
            \label{fig:kather_10NN_13}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/56/2.png}
            \label{fig:kather_10NN_14}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/56/3.png}
            \label{fig:kather_10NN_15}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/56/4.png}
            \label{fig:kather_10NN_16}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/56/5.png}
            \label{fig:kather_10NN_17}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/56/6.png}
            \label{fig:kather_10NN_18}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/56/7.png}
            \label{fig:kather_10NN_19}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/56/8.png}
            \label{fig:kather_10NN_20}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/56/9.png}
            \label{fig:kather_10NN_21}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/56/10.png}
            \label{fig:kather_10NN_22}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/72/instance.png}
            \label{fig:kather_10NN_23}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/72/1.png}
            \label{fig:kather_10NN_24}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/72/2.png}
            \label{fig:kather_10NN_25}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/72/3.png}
            \label{fig:kather_10NN_26}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/72/4.png}
            \label{fig:kather_10NN_27}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/72/5.png}
            \label{fig:kather_10NN_28}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/72/6.png}
            \label{fig:kather_10NN_29}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/72/7.png}
            \label{fig:kather_10NN_30}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/72/8.png}
            \label{fig:kather_10NN_31}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/72/9.png}
            \label{fig:kather_10NN_32}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/72/10.png}
            \label{fig:kather_10NN_33}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/18/instance.png}
            \label{fig:kather_10NN_34}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/18/1.png}
            \label{fig:kather_10NN_35}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/18/2.png}
            \label{fig:kather_10NN_36}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/18/3.png}
            \label{fig:kather_10NN_37}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/18/4.png}
            \label{fig:kather_10NN_38}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/18/5.png}
            \label{fig:kather_10NN_39}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/18/6.png}
            \label{fig:kather_10NN_40}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/18/7.png}
            \label{fig:kather_10NN_41}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/18/8.png}
            \label{fig:kather_10NN_42}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/18/9.png}
            \label{fig:kather_10NN_43}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/18/10.png}
            \label{fig:kather_10NN_44}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/189/instance.png}
            \label{fig:kather_10NN_45}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/189/1.png}
            \label{fig:kather_10NN_46}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/189/2.png}
            \label{fig:kather_10NN_47}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/189/3.png}
            \label{fig:kather_10NN_48}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/189/4.png}
            \label{fig:kather_10NN_49}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/189/5.png}
            \label{fig:kather_10NN_50}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/189/6.png}
            \label{fig:kather_10NN_51}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/189/7.png}
            \label{fig:kather_10NN_52}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/189/8.png}
            \label{fig:kather_10NN_53}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/189/9.png}
            \label{fig:kather_10NN_54}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/189/10.png}
            \label{fig:kather_10NN_55}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/318/instance.png}
            \label{fig:kather_10NN_56}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/318/1.png}
            \label{fig:kather_10NN_57}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/318/2.png}
            \label{fig:kather_10NN_58}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/318/3.png}
            \label{fig:kather_10NN_59}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/318/4.png}
            \label{fig:kather_10NN_60}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/318/5.png}
            \label{fig:kather_10NN_61}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/318/6.png}
            \label{fig:kather_10NN_62}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/318/7.png}
            \label{fig:kather_10NN_63}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/318/8.png}
            \label{fig:kather_10NN_64}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/318/9.png}
            \label{fig:kather_10NN_65}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/318/10.png}
            \label{fig:kather_10NN_66}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/322/instance.png}
            \label{fig:kather_10NN_67}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/322/1.png}
            \label{fig:kather_10NN_68}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/322/2.png}
            \label{fig:kather_10NN_69}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/322/3.png}
            \label{fig:kather_10NN_70}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/322/4.png}
            \label{fig:kather_10NN_71}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/322/5.png}
            \label{fig:kather_10NN_72}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/322/6.png}
            \label{fig:kather_10NN_73}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/322/7.png}
            \label{fig:kather_10NN_74}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/322/8.png}
            \label{fig:kather_10NN_75}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/322/9.png}
            \label{fig:kather_10NN_76}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/322/10.png}
            \label{fig:kather_10NN_77}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/262/instance.png}
            \label{fig:kather_10NN_78}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/262/1.png}
            \label{fig:kather_10NN_79}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/262/2.png}
            \label{fig:kather_10NN_80}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/262/3.png}
            \label{fig:kather_10NN_81}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/262/4.png}
            \label{fig:kather_10NN_82}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/262/5.png}
            \label{fig:kather_10NN_83}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/262/6.png}
            \label{fig:kather_10NN_84}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/262/7.png}
            \label{fig:kather_10NN_85}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/262/8.png}
            \label{fig:kather_10NN_86}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/262/9.png}
            \label{fig:kather_10NN_87}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/262/10.png}
            \label{fig:kather_10NN_88}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/77/instance.png}
            \label{fig:kather_10NN_89}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/77/1.png}
            \label{fig:kather_10NN_90}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/77/2.png}
            \label{fig:kather_10NN_91}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/77/3.png}
            \label{fig:kather_10NN_92}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/77/4.png}
            \label{fig:kather_10NN_93}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/77/5.png}
            \label{fig:kather_10NN_94}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/77/6.png}
            \label{fig:kather_10NN_95}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/77/7.png}
            \label{fig:kather_10NN_96}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/77/8.png}
            \label{fig:kather_10NN_97}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/77/9.png}
            \label{fig:kather_10NN_98}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/77/10.png}
            \label{fig:kather_10NN_99}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/223/instance.png}
            \label{fig:kather_10NN_100}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/223/1.png}
            \label{fig:kather_10NN_101}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/223/2.png}
            \label{fig:kather_10NN_102}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/223/3.png}
            \label{fig:kather_10NN_103}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/223/4.png}
            \label{fig:kather_10NN_104}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/223/5.png}
            \label{fig:kather_10NN_105}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/223/6.png}
            \label{fig:kather_10NN_106}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/223/7.png}
            \label{fig:kather_10NN_107}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/223/8.png}
            \label{fig:kather_10NN_108}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/223/9.png}
            \label{fig:kather_10NN_109}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/223/10.png}
            \label{fig:kather_10NN_110}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/225/instance.png}
            \label{fig:kather_10NN_111}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/225/1.png}
            \label{fig:kather_10NN_112}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/225/2.png}
            \label{fig:kather_10NN_113}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/225/3.png}
            \label{fig:kather_10NN_114}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/225/4.png}
            \label{fig:kather_10NN_115}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/225/5.png}
            \label{fig:kather_10NN_116}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/225/6.png}
            \label{fig:kather_10NN_117}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/225/7.png}
            \label{fig:kather_10NN_118}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/225/8.png}
            \label{fig:kather_10NN_119}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/225/9.png}
            \label{fig:kather_10NN_120}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/NearestNeighbours/225/10.png}
            \label{fig:kather_10NN_121}
        \end{subfigure}
    \caption[]
    {Some captions}
    \label{fig:label}
\end{figure*}


==> Texfiles_ToInput/Kather/kather_10NN_0_6_mainarticle.tex <==
\begin{figure*}
    \captionsetup[subfigure]{labelformat=empty}
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/11/instance.png}
            \label{fig:kather_10NN_1}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/11/1.png}
            \label{fig:kather_10NN_2}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/11/2.png}
            \label{fig:kather_10NN_3}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/11/3.png}
            \label{fig:kather_10NN_4}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/11/4.png}
            \label{fig:kather_10NN_5}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/11/5.png}
            \label{fig:kather_10NN_6}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/11/6.png}
            \label{fig:kather_10NN_7}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/11/7.png}
            \label{fig:kather_10NN_8}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/11/8.png}
            \label{fig:kather_10NN_9}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/11/9.png}
            \label{fig:kather_10NN_10}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/11/10.png}
            \label{fig:kather_10NN_11}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/24149/instance.png}
            \label{fig:kather_10NN_12}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/24149/1.png}
            \label{fig:kather_10NN_13}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/24149/2.png}
            \label{fig:kather_10NN_14}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/24149/3.png}
            \label{fig:kather_10NN_15}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/24149/4.png}
            \label{fig:kather_10NN_16}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/24149/5.png}
            \label{fig:kather_10NN_17}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/24149/6.png}
            \label{fig:kather_10NN_18}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/24149/7.png}
            \label{fig:kather_10NN_19}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/24149/8.png}
            \label{fig:kather_10NN_20}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/24149/9.png}
            \label{fig:kather_10NN_21}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/24149/10.png}
            \label{fig:kather_10NN_22}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/12062/instance.png}
            \label{fig:kather_10NN_23}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/12062/1.png}
            \label{fig:kather_10NN_24}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/12062/2.png}
            \label{fig:kather_10NN_25}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/12062/3.png}
            \label{fig:kather_10NN_26}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/12062/4.png}
            \label{fig:kather_10NN_27}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/12062/5.png}
            \label{fig:kather_10NN_28}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/12062/6.png}
            \label{fig:kather_10NN_29}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/12062/7.png}
            \label{fig:kather_10NN_30}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/12062/8.png}
            \label{fig:kather_10NN_31}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/12062/9.png}
            \label{fig:kather_10NN_32}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/12062/10.png}
            \label{fig:kather_10NN_33}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/28935/instance.png}
            \label{fig:kather_10NN_34}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/28935/1.png}
            \label{fig:kather_10NN_35}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/28935/2.png}
            \label{fig:kather_10NN_36}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/28935/3.png}
            \label{fig:kather_10NN_37}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/28935/4.png}
            \label{fig:kather_10NN_38}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/28935/5.png}
            \label{fig:kather_10NN_39}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/28935/6.png}
            \label{fig:kather_10NN_40}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/28935/7.png}
            \label{fig:kather_10NN_41}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/28935/8.png}
            \label{fig:kather_10NN_42}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/28935/9.png}
            \label{fig:kather_10NN_43}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/28935/10.png}
            \label{fig:kather_10NN_44}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/27219/instance.png}
            \label{fig:kather_10NN_45}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/27219/1.png}
            \label{fig:kather_10NN_46}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/27219/2.png}
            \label{fig:kather_10NN_47}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/27219/3.png}
            \label{fig:kather_10NN_48}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/27219/4.png}
            \label{fig:kather_10NN_49}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/27219/5.png}
            \label{fig:kather_10NN_50}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/27219/6.png}
            \label{fig:kather_10NN_51}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/27219/7.png}
            \label{fig:kather_10NN_52}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/27219/8.png}
            \label{fig:kather_10NN_53}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/27219/9.png}
            \label{fig:kather_10NN_54}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/27219/10.png}
            \label{fig:kather_10NN_55}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/16479/instance.png}
            \label{fig:kather_10NN_56}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/16479/1.png}
            \label{fig:kather_10NN_57}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/16479/2.png}
            \label{fig:kather_10NN_58}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/16479/3.png}
            \label{fig:kather_10NN_59}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/16479/4.png}
            \label{fig:kather_10NN_60}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/16479/5.png}
            \label{fig:kather_10NN_61}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/16479/6.png}
            \label{fig:kather_10NN_62}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/16479/7.png}
            \label{fig:kather_10NN_63}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/16479/8.png}
            \label{fig:kather_10NN_64}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/16479/9.png}
            \label{fig:kather_10NN_65}
        \end{subfigure}
\hfill
    \centering
        \begin{subfigure}[b]{0.08636363636363636\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/NearestNeighbours/16479/10.png}
            \label{fig:kather_10NN_66}
        \end{subfigure}
    \caption[]
    {Some captions}
    \label{fig:kather_10NN}
\end{figure*}

==> Texfiles_ToInput/camlike_mainarticle.tex <==
\begin{figure*}
    \captionsetup[subfigure]{labelformat=empty}
    \centering
        \begin{subfigure}[b]{0.95\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/MNIST/CAMlike/110.png}
            \label{fig:camlike_1}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.95\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/CAMlike/11.png}
            \label{fig:camlike_2}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.95\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/Kather/CAMlike/18655.png}
            \label{fig:camlike_3}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.95\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/CAMlike/45.png}
            \label{fig:camlike_4}
        \end{subfigure}
\\
    \centering
        \begin{subfigure}[b]{0.95\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/DogsWolves/CAMlike/225.png}
            \label{fig:camlike_5}
        \end{subfigure}
    \caption[]
    {Some captions sdf.}
    \label{fig:camlike}
\end{figure*}

==> Transactions-Bibliography/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************

